Dataset search: a survey

Generating value from data requires the ability to find, access and make sense of datasets. There are many efforts underway to encourage data sharing and reuse, from scientific publishers asking authors to submit data alongside manuscripts to data marketplaces, open data portals and data communities. Google recently beta released a search service for datasets, which allows users to discover data stored in various online repositories via keyword queries. These developments foreshadow an emerging research field around dataset search or retrieval that broadly encompasses frameworks, methods and tools that help match a user data need against a collection of datasets. Here, we survey the state of the art of research and commercial systems in dataset retrieval. We identify what makes dataset search a research field in its own right, with unique challenges and methods and highlight open problems. We look at approaches and implementations from related areas dataset search is drawing upon, including information retrieval, databases, entity-centric and tabular search in order to identify possible paths to resolve these open problems as well as immediate next steps that will take the field forward.

==> currenttech.tex <==
\section{Gems to consider} \label{sec:currenttech}

EXPLAIN WHY THESE AREAS ARE RELEVANT AND NOT OTHERS. EXPLAIN HOW THEY ARE RELATED AND WHETHER THE TERMINOLOGY IS USED CONSISTENLY. 

YOU'RE MISSING QUESTION ANSWERING. EVEN IF YOU DON'T COVER IT, I WOULD EXPLAIN WHY IT IS NOT RELEVANT.

WE'RE ALSO MISSING OUR DEFINITION OF A DATASET AND OF THE DATASET SEARCH PROBLEM.

Search has been addressed across many computer science sub-disciplines, such as databases, information retrieval, entity-centric search and tabular search. Figure \ref{fig:searchoverview} contains an overview of the high-level steps, and how each sub-discipline implements them. While dataset search is a subject in its own right, with distinct challenges and characteristics, it shares commonalities and draws upon insights from all these areas. In this section, we highlight related research that has already been, or could be, co-opted by dataset search. In particular, we would like to highlight the gems that could be used to address the Open Problems highlighted in Section \ref{sec:openproblems}. 

 \subsection{Entity-centric search}
% \TODO{Do you have anything special to say in this section about: Metadata; Schemas; Data Quality; Data profiling; Provenance; Annotation; Licenses}
% Can be said, but unsure if ti wouldn't add a lot of clutter.
The semantic web community has worked towards creating machine-understandable graph-based representations of data \cite{ldbook}. It proposes languages, models and techniques to publish data online in the form of entities, properties, literals, and, most importantly, links to other resources. These links facilitate search and exploration of a global decentralized data space, similar to browsing and navigation on the web. The World Wide Web Consortium (W3C) settled on the Resource Description Format (RDF) as a standard model for representing and exchanging data about resources, which can refer to conventional web content as well as entities in the offline world such as people, places and organizations, identified by \emph{International Resource Identifiers} (IRIs). Properties link entities or attach attributes to them. By reusing and linking IRIs, publishers signal that they hold data about the same entity, therefore enabling queries such as \emph{Who holds data about England?} and \emph{What do you know about England?} across multiple resources without any additional integration effort. 

Realising the web of data requires several steps: lifting existing data into the semantic web, commonly referred to as linked (open) data \cite{ldcycle}, defining vocabularies and schemas to describe data in RDF and connecting to other datasets. For example, the Linked Open Vocabulary portal\footnote{\url{https://lov.linkeddata.es}} lists $635$ such vocabularies, and provides search and exploration capabilities to find commonly used IRIs, to assist publishers in reusing them to facilitate data interpretation and interlinking. 

Interlinking comprises two complementary problems. First is \emph{entity resolution}: given two or more datasets, identify which entities and properties are the same. A general framework of entity resolution is described \cite{erbook}. It covers the design of \emph{similarity metrics} to compare entity descriptions, and the development of \emph{blocking} techniques to group roughly similar entities together, in order to not apply more expensive similarity metrics to entities that have a low chance of ultimately resolving to the same entity. Finally, more recent efforts have tried \emph{iterative} approaches, where discovered matches are used as input for computing similarities between further entities. The second part of interlinking is referred to as \emph{link discovery}, where given two datasets, one has to find properties that hold between their entities. Properties can be equivalence or equality, as in entity resolution, or domain specific such as 'part-of' \cite{linkingsurvey}.

%Next, a number of researchers have tackled the problem of maintaining and repairing the links, that is, to answer the question \emph{What happens with links whenever a link disappears}. Indeed, with respect to the traditional Distributed Database setting, where all servers are under the control of a single organisation, in a Web environment each server is controlled by different autonomous organisations that might update their servers unexpectedly 

%Once datasets are published and linked, the next step is to evaluate and assure the quality of the links. \cite{zaveri2016quality} provides an in-depth review of quality assurance methods for linked data. 

Querying linked data can be done via languages such as SPARQL, a W3C recommendation. In a similar way to a distributed database, given a query $Q$ and a set of RDF datasets (the \emph{sources}), the query engine first selects the datasets relevant to the query~\cite{saleem_hibiscus:_2014,vidal_selection_2016} and then chooses between different approaches: aggregating the datasets locally, using distributed processing as in Hadoop~\cite{wylot_rdf_2018}, or a federated approach~\cite{oguz_federated_2015}. 

One can apply the Linked Data paradigm to solve dataset search by converting datasets to RDF and following the full cycle, as described in~\cite{kunze_dataset_2013}. However, for data publishers, it is often still very expensive to execute the full cycle. Furthermore, there is debate on whether certain datasets should have an RDF representation at all, as their original formats are perhaps more suited to the tools that are required for them (e.g. geospatial datasets). A middle-ground solution is to consider datasets as resources and encode only their description in RDF, for example, using the Data Catalog Vocabulary (a W3C recommendation)~\cite{dcat}. Then, the Linked Data cycle can then be applied to these descriptions, ultimately enabling the querying of datasets. The main challenge is the generation and maintenance of these descriptions, with some works tackling the problem of extracting specific properties from specific formats, like ~\cite{neumaier2018enabling} for extracting spatio-temporal properties, and \cite{kacprzak_making_2018} for identifying the numerical properties in CSV tables.

ADD ENTITY CENTRIC SEARCH HERE, MORE RELEVANT IN MY OPINION THAN RDF AND LINKED DATA

%\TODO{Add more on querying}. \cite{Bailey:2005:WSW:2156061.2156064,FIKES200419,mcbride:2002,KAUFMANN2010377,xiao:2018,Sakr2018} possibly.

\subsection{Information retrieval} \label{sec:ir}
THIS IS THE WEAKEST SUBSECTION, IT DOES NOT OFFER ENOUGH INSIGHT INTO RECENT, ADVANCED WORK. IT IS AT THE LEVEL OF AN UNDERGRAD COURSE OR A WIKIPEDIA PAGE.
%[Emilia] Information Retrieval and what could be applied from it. Most portals use the IR based because indexing the text of the description. Only slowly moving to publishing as DCAT, which is now picked up. \\
The main purpose of an information retrieval (IR) system is to aid users in the process of finding information of their interest \cite{baeza2011modern}. IR systems can be broadly classified in web and document search engines, and engines for other types of entities (images, people, etc), called \emph{vertical search engines}.
%Depending of the underlying resources information retrieval algorithms are adapted to maximise their efficiency. 
The web and document engines use a number of statistical techniques to compute the relevance of a word (coming from an user query) to a document. The most established of such techniques is TF-IDF \cite{zhang2008tfidf}. In addition to relevance functions like TF-IDF, web search engines take advantage of the hyper-linked structure of the web. The basic premise follows the idea that each web page can be modelled as a node of a directed graph, with hyperlinks as edges, and that the more edges pointing towards a document, the more relevant it is. The most well known implementation of this concept is the Page-Rank algorithm ~\cite{brin2012reprint,page1999pagerank}.
%Based on the model of the web generated by crawlers, which map each web page following the links, an index of resources is created to rank resources relevant to the user query \cite{croft2010search}. 
Further improvements to ranking functions include machine learning models \cite{Agichtein:2006:LUI:1148170.1148175}, personalisation of results, \cite{Sieg:2007:WSP:1321440.1321515} and providing question answering capabilities \cite{Kwok:2001:SQA:502115.502117}.

Vertical search engines are specifically tailored to the characteristics of the resources. For example, an email search has unique sets of  resources for each users in addition to specific metadata such as sender and receiver addresses, topic or timestamp in order to judge the relevance \cite{Ai:2017:CES:3038912.3052615}. Another vertical search example, publication search, uses the publication year, list of authors, conference or journal importance factor as well as list of keywords \cite{Li2010,Yu:2005:ATD:1092358.1092535}. Due to the specificity and limited scope of resources, vertical search engines often offer greater precision, utilize more complex schemas to match specific searching scenarios, and tend to support more complex user tasks \cite{Li2010,Yu:2005:ATD:1092358.1092535}.
%People search \citep{Weerkamp2011peoplesearch, guy2012best} is gaining more importance with portals like LinkedIn or Facebook.

% Open data portals are a point of free access to the governmental and institutional data for both commercial and non-commercial purposes through cataloguing with common metadata, which allow search and explorative activities.

THIS IS AN IMPLEMENTATION?
Well-known information retrieval techniques are currently applied to the problem of dataset retrieval, on open data platforms.

In the context of dataset retrieval the basic concepts supporting  general web search are not sufficient, which indicates a need for more targeted approach for dataset retrieval, treating it as a unique vertical \cite{Cafarella:2008:WEP:1453856.1453916,Gonzalez:2010:GFT:1807167.1807286}. 
As pointed out by Cafarella et al. \cite{Cafarella:2008:WEP:1453856.1453916} structured data on the web is similar to the scenario of ranking of millions of individual databases. Tables available online contain a mixture of structural and related content elements which cannot easily be mapped to unstructured text scenarios applied in general web search. Tables lack the incoming hyperlink anchor text and are two-dimensional - they cannot be efficiently queried using the standard inverted index. For those reasons PageRank-based algorithms known from general web search are not applicable to the same extend to the dataset/table search, particularly as tables of widely-varying quality can be found on a single web page.
%Fusion tables, google base?, bio sciences, health data, database search, product search,

%In Section \ref{sec:googleimpl} we present in more detail approaches that were proposed to facilitate the search for datasets.

\subsection{Databases} \label{sec:databases}
Traditionally, the database community has focused on the management, search and retrieval of data within a database; in this section we highlight several areas in which work within the database community could be utilized by dataset search. 

The classic pipeline for search within a database begins with a structured query. The database community has a long-standing and rich history of structured query languages beginning with SEQUEL for the R database \cite{Chamberlin:1976,Chamberlin:1974:SSE:800296.811515,Negri:1991:FSS:111197.111212}. Structured query languages have been explored for relational \cite{Buneman:1982:ITD:319702.319711,melton:2002} as well as many semi-structured data types such as XML \cite{DEUTSCH19991155}, RDF \cite{Haase:2004} through to graphs \cite{Angles:2018:GCF:3183713.3190654}.  Each of these languages have been created to take into account the requirements of the data within that format. Querying datasets will likely require new adaptations and methods. The overlap of programming languages and database query languages \cite{cheney_grust_2018} in which programming language concepts are used to define queries over databases with different levels of capabilities \cite{seco:2017} or over MapReduce frameworks \cite{fegaras:2017}, could be one such rich area to explore.  

As with query languages, there is a rich and long-history in query processing \cite{Catania2018}. Once a query is issued, the classic pipeline includes: parsing the query \cite{Chen:2000:NSC:342009.335432,Li:2005:NIN:1066157.1066281}; creating an evaluation plan \cite{Levy1995}; optimizing the plan \cite{Chaudhuri:1998:OQO:275487.275492,Ioannidis:1996:QO:234313.234367}; executing the plan utilizing appropriate indexes and catalogues \cite{bertino:2012}. The relational algebra that underpins our processing within a database \cite{codd1972relational}, has no equivalent yet in dataset search. Recently, Apache released information about the query processing system used for many of the Apache products including Hive and Storm, and  \cite{Begoli:2018:ACF:3183713.3190662} investigated how the relational algebra can be applied to data contained within the various data processing frameworks in the Apache suite. Alternatively, other recent work in query processing attempts to handle non-relational operators via adaptive query processing \cite{kaftan:2018}.

\noindent \textbf{Data integration} is the problem of combining information from
multiple, distributed, and heterogeneous sources. The need to integrate data is ubiquitous across domains, including for creating vertical dataset search engines (see Section \ref{sec:deepweb}), and for providing solutions to the constructive dataset search problem (see Example \ref{ex:constructive}).  While the last 15 years have seen significant progress on the theory of data integration
\cite{arenas2010,fagin2005,genesereth2010halevy2001,lenzerini2002};
much work is still needed to achieve practical solutions that can
scale to the size required by contemporary problems. Many sub-problems raise specific challenges: source discovery
\cite{bhagat2010,Cafarella:2008:WEP:1453856.1453916,dong2004,Gonzalez:2010:GFT:1807167.1807286},
source modeling and schema mapping
\cite{alexe2011,Bellahsene:2011:SMM:1972526,doan2003,fagin2009,clio,rahm01,massmann2011,shvaiko05},
and querying the sources in an integrated fashion
\cite{arenas2010,duschka2000:jlp,fagin2005,genesereth2010,halevy2001,konstantinidis2011,lenzerini2002}.

From a architectural perspective, data integration can be accomplished
through data warehousing or virtual integration. In the {\em
  warehouse} approach, the integrator cleans, reconciles and
materializes (loads) the data from the sources into a single data
repository (e.g., a relational database).  In the {\em virtual
  integration} approach, the data remains at the original sources and
the system accesses and integrates the data from the sources in
response to user queries in real time.
%
These approaches have complementary properties. The warehouse
approach provides more efficient query answering for queries that
require large amounts of data to be processed simultaneously.
However, the data in the warehouse may become stale; it is only as
recent as the last update cycle.  The virtual integration approach
always accesses the latest data from the sources, so it is necessary
when data is updated often, when having the latest data is critical,
or when organizational or legal constraints prevent the
incorporation of data sources into a warehouse.
%
These two approaches are not mutually exclusive. Some data can be
materialized locally and some accessed at run-time from remote
sources.
%

\noindent \textbf{Data profiling and data quality} facilitate understanding the 'shape' of a dataset. As noted in \cite{bailis2017}, users do not have the 'attention' to introspect deeply into large and changing datasets. Instead, we can draw upon several areas of research from the database community, including data profiling and data quality. 

Naumann's recent survey \cite{Naumann:2014:DPR:2590989.2590995} provides a good overview of data profiling activities based on how data-users approach the task, and what resources are available for it.  Of particular note for dataset search is the work on outlier detection \cite{dong2017authenticated,DBLP:conf/sigmod/LiuJ09} as a way to provide indications to an end-user about the scope, spread and variety of a dataset during search. In particular, we note the techniques found in  \cite{Zhang:2016:SEE:3021924.3021928} are interesting for dataset search in that they split a large dataset into many smaller datasets and create an approximate representation of it for more accurate sampling of these sub-pieces.  Finally, \cite{Gao:2018:NDL:3183713.3183746} establishes a tool that can comb through semi-structured log datasets to pull information into multi-layered structured datasets. All of these techniques may aid users in exploring and making sense of dataset.

The work on profiling  contains expressions of data cleanliness and coverage, completeness and consistency. These properties are classic data quality metrics, and help the user form a picture of whether the data is fit for use. Automatic understanding of data quality in order to either populate metadata or answer metadata queries in a lazy manner will require techniques that can automatically determine complex datatypes such as \cite{Yan:2018:STL:3183713.3196888}. Currently, though, the research in each of these areas has been focused on its relationship to describing or working within a specific artifact, not as a component for a search. To do this, the structures and content for each area need to be computable in a timely manner and presented in a way that can be taken advantage of by a search system. For instance, data quality is a traditionally resource expensive task that is often domain-specific. Generic, albeit possibly less accurate methods must be developed to compute data quality estimations that can be accessed and used during search \cite{Chapman:2016:CLD:2888577.2834123,missier:2006}. Techniques such as those found in \cite{Peng:2018:ACA:3183713.3183747} suggest using a hybrid version of approximate query processing over samples and precomputation. Solutions such as ORCHESTRA \cite{Ives:2008:OCD:1462571.1462577} that were built to manage shared, structured data with changing schemas, cleaning, and queries that utilize provenance and annotation information (discussed in more detail below) need to be adapted to the dataset search problem. 

\noindent {\bf Summarization, provenance and annotation} are all additional types of metadata that have been studied within the database community, and may facilitate dataset search. In order to assist users to identify and understand a dataset without introspection of the dataset, summarization can be used, as done in \cite{Orr:2017:PDS:3115404.3115419} over probabilistic databases. Other work from the probabilistic database area could also be of assistance. For instance \cite{dylla:2013} calculates the top-k results for queries over a probabilistic database by taking into account the lineage of each tuple. This usage of provenance to influence the overall ranking of the end result could inform dataset ranking. In a similar vein, provenance \cite{Buneman:2006:PMC:1142473.1142534,Green:2007:PS:1265530.1265535,DBLP:journals/vldb/HerschelDL17,wylot2017storing} is likely to be a key element in assisting the user in choosing a dataset of interest. Until now, provenance has been used to facilitate trust in an artifact \cite{CURCIN20171,dai:2008} or automatically estimate quality \cite{huynh:2018}. At least three expansions in this area need to be undertaken in order to fully utilize provenance for dataset search. First, provenance is a record of history - new methods must be developed to facilitate translation of this large graph into a format that a user who is evaluating whether or not to use a dataset can interpret and utilize \cite{chapman:2011}. Second, one could expand the work of \cite{dylla:2013} in which top-k tuples are ranked by using lineage, and instead rank datasets using provenance and the criteria of the searcher. Third, there is an unsolved problem of moving across granularity levels in provenance. A tuple within a dataset may have provenance associated with it, as may the table, and the entire dataset itself. The challenge is in understanding how the aggregation of tuple-provenance would affect the search results compared to dataset-provenance.  Overall, the entire logic behind dataset search will open up new areas for determining why and why  not to consider provenance of the dataset query results themselves \cite{Chapman:2009:WHY:1559845.1559901,cheney:2009,DBLP:journals/vldb/HerschelDL17,lee:2017}

Annotations have a different set of functions and research problems within dataset search. In this case, annotations on datasets are already used to facilitate search results \cite{Geerts06mondrian:annotating,KIRYAKOV200449}. Current annotation work such as summarizing annotations \cite{Xiao:2015:EMG:2723372.2735355}, or  using annotations to improve the data \cite{Ibrahim:2015:PAM:2723372.2749435} will be needed. Interesting extensions could include using user feedback to facilitate ranking of datasets based on the searcher's criteria, or utilizing the context under which the annotations were created to change how annotations impact ranking.   Finally, with respect to constructive dataset search (see \ref{ex:constructive}), the work of \cite{Wu:2018:DCG:3183713.3196910} is essential to appropriately annotate and cite the results of queries.

\input{hiddenweb.tex}

\input{tabularsearch.tex} 
